On the use of feature-maps and parameter control for improved quality-diversity meta-evolution

In Quality-Diversity (QD) algorithms, which evolve a behaviourally diverse archive of high-performing solutions, the behaviour space is a difficult design choice that should be tailored to the target application. In QD meta-evolution, one evolves a population of QD algorithms to optimise the behaviour space based on an archive-level objective, the meta-fitness. This paper proposes an improved meta-evolution system such that (i) the database used to rapidly populate new archives is reformulated to prevent loss of quality-diversity; (ii) the linear transformation of base-features is generalised to a feature-map, a function of the base-features parametrised by the meta-genotype; and (iii) the mutation rate of the QD algorithm and the number of generations per meta-generation are controlled dynamically. Experiments on an 8-joint planar robot arm compare feature-maps (linear, non-linear, and feature-selection), parameter control strategies (static, endogenous, reinforcement learning, and annealing), and traditional MAP-Elites variants, for a total of 49 experimental conditions. Results reveal that non-linear and feature-selection feature-maps yield a 15-fold and 3-fold improvement in meta-fitness, respectively, over linear feature-maps. Reinforcement learning ranks among top parameter control methods. Finally, our approach allows the robot arm to recover a reach of over 80% for most damages and at least 60% for severe damages.

==> paper/discussion.tex <==
%\section{Discussion}

% -P1: restate the key points


%parameter control

%Our parameter control investigations provide a few recommendations. For linear feature-maps, both the mutation rate and the number of generations benefit from reinforcement learning control. For non-linear feature-maps, high mutation rates and low number of generations of meta-generations are observed to be beneficial for meta-fitness. Lower number of generations imply more frequent meta-fitness evaluation and therefore the space of feature-maps is more widely explored. High mutation rates  exploratio

%High mutation rates are typically preferable for improving the meta-fitness, possibly because MAP-Elites finds elites concentrated in particular regions of the genotypic space and increased mutation rates help to discover other genotypic regions. \textbf{Does this mimic Nordmoen et al?} The number of generations per meta-generation should be set relatively low to ensure improvement of meta-fitness within the budget of function evaluations. For the budget of 100 million function evaluations, the lowest included setting of 5 generations converged rapidly to the maximal observed meta-fitness although it is not known whether other conditions could make further improvements to the meta-fitness. 

% 
%For dynamic parameter control, ... 
%
%We also find that assessing behavioural diversity versus behavioural diversity over damages is comparable.and environmental diversity are strongly related, as noted in \cite{Bossens2020b}, such that performance across a wide set of damages is similar to performance across a wide set of behaviours.  

% P2: Discuss recommendations/implications based on our results


% P2b recommendations based on parameter control
%Endogenous approach may not work well for meta-evolution of the number of bottom-level generations; because the meta-fitness does not take into account the number of function evaluations that have passed, the algorithm finds that it optimises the meta-fitness by allowing many bottom-level generations but does not take into account that it can do fewer meta-generations. By contrast, the reward in the reinforcement learning approach divides by the number of evaluations that have passed.
%
%To extend the parameter control to other parameters or to different domains, one must, however, consider the wider applicability of the endogenous and the RL approach. Endogenous and RL methods can adapt the parameter control strategy to the domain and parameter and can therefore be applied generically. By contrast, annealing and static settings are parameter- and domain-specific. Annealing, or linearly decreasing the parameter, is expected to work as a heuristic specifically for mutation rate and number of iterations due to the need for exploration and solution generation at the start of the algorithm and the need for exploitation and solution testing at the end of the algorithm; annealing is not expected to work for other parameters. Furthermore, annealing may not always perform well, even when one would expect it to do so, and in this case there is no adaptivity in the annealing strategy to recover. A static parameter choice ignores the dynamic changes that may be needed during the course of evolution and even if no such changes are required, the best static setting would still need to be found by manual tuning rather than automated evolution or RL.

% P3 : how our approach departs from other automated approaches --> meta-evoluttion
%
%Nordmoen et al. (2018) \cite{Nordmoen2018} explore various static and dynamic schemes for the mutation rate in traditional MAP-Elites. In designing behaviour primitives for quadruped robots, they show that generally there is a positive effect of dynamic schemes and that there is a trade-off for endogenous parameter control, where results are more consistent but with a lower upper bound to performance . 

%-P4: limitations, possible improvements, future
% 

